On VLMs for Diverse Tasks in Multimodal Meme Classification

In this paper, we present a comprehensive and systematic analysis of vision-language models (VLMs) for disparate meme classification tasks. We introduced a novel approach that generates a VLM-based understanding of meme images and fine-tunes the LLMs on textual understanding of the embedded meme text for improving the performance. Our contributions are threefold: (1) Benchmarking VLMs with diverse prompting strategies purposely to each sub-task; (2) Evaluating LoRA fine-tuning across all VLM components to assess performance gains; and (3) Proposing a novel approach where detailed meme interpretations generated by VLMs are used to train smaller language models (LLMs), significantly improving classification. The strategy of combining VLMs with LLMs improved the baseline performance by 8.34%, 3.52% and 26.24% for sarcasm, offensive and sentiment classification, respectively. Our results reveal the strengths and limitations of VLMs and present a novel strategy for meme understanding.

==> latex/20RelatedWorks.tex <==
\section{Related Works:}

% \subsection{Datasets for meme emotion detection:}

% \subsection{Methods for meme emotion detection:}

% \subsection{Methods for meme understanding:}

% Researchers explored various AI models to perform diverse tasks from multi-modal memes and developed diverse datasets\cite{xu2022met}. \textcolor{blue}{mention which works presented new dl models, which works used VLMs. mention that the details are given in the appendix section.}

%Among these works, Xu et al.\cite{xu2022met} introduced the MET-Meme dataset to interpret memes with metaphors in the multi-modal framework of memes. Liu et al. \cite{liu2022figmemes} presented a new multi-modal learning model called FigMemes, which focused on figurative language identification tasks such as annotations for sarcasm, irony, metaphor, and hyperbole, crucial for understanding nuanced political messages. Pan et al. \cite{pan2020modeling} proposed a multi-modal sarcasm detection framework for modeling incongruities within and between text and images. The work utilized intra-modal and inter-modal attention mechanisms to effectively capture the subtle sarcastic cues in memes, highlighting the importance of multimodal information. Suryawanshi et al. \cite{suryawanshi2020multimodal} created the MultiOFF dataset, which identifies offensive memes by incorporating emotional components such as sarcasm and satire. The work attempts to distinguish different forms of offensive language within visual contexts and highlights the importance of cultural and linguistic diversity. Fersini et al. \cite{fersini2022semeval} created a dataset that serves as a benchmark for identifying misogynistic memes. The work encompasses tasks for classifying such content and categorizing it into specific behaviors. Ramamoorthy et al. \cite{ramamoorthy2022memotion} proposed a new framework termed DISARM, which detects entities targeted by harmful content in memes by integrating multi-modal features with named entity recognition. Zhong et al. \cite{zhong2024multimodal} analyzed memes to study the presence of bias and fairness of these VLMs for meme understanding, such as LLaVA 1.5 and MiniGPT-4 to classify and comprehend memes. The work also studied other important aspects, such as bias and fairness of these VLMs for meme understanding. 

% The recent interest in multimodal meme analysis has led to the development of several multimodal datasets (containing text and image) focusing on diverse tasks. While the area has made rapid strides, several challenges, such as role effective feature extraction, adoption of transfer learning, understanding the rationale behind the predictions, robustness, and generalizability of the models, remain. Addressing these challenges will help the models perform well in controlled settings and adapt to the continuously evolving landscape of online meme culture.

%The research in multi-modal meme analysis has introduced innovative datasets and modeling techniques that effectively leverage the integration of visual and textual modalities. While the field has made strides in improving model accuracy through innovative feature extraction and the adoption of transfer learning, challenges remain. Issues related to computational complexity, model interpretability, real-world robustness, and the integration of external context highlight the need for further research. Addressing these challenges will be crucial for developing models that not only perform well in controlled environments but also adapt effectively to the continuously evolving landscape of online meme culture.



Several recent works attempted to analyze memes using either custom DL models or VLMS. Besides, X number of datasets and Y number of high-quality publications have been published in the last 5 years. A detailed discussion of these models, datasets, and approaches is provided in the Appendix (Section~\ref{relatedwork}).

% such as FigMemes for figurative language identification~\cite{liu2022figmemes}, multimodal sarcasm detection using attention mechanisms~\cite{pan2020modeling}, and DISARM for harmful entity detection~\cite{ramamoorthy2022memotion}. Vision-Language Models (VLMs) like LLaVA 1.5 (LV) and MiniGPT-4 (MG) have also been evaluated for meme classification and bias analysis~\cite{zhong2024multimodal}. Additionally, multimodal datasets have been introduced to support these tasks, including MET-Meme~\cite{xu2022met}, MultiOFF~\cite{suryawanshi2020multimodal}, and a misogynistic meme benchmark~\cite{fersini2022semeval}. A detailed discussion of these models, datasets, and approaches is provided in the Appendix (Section~\ref{relatedwork}).
